Probing the Moral Development of Large Language Models through Defining Issues Test

In this study, we measure the moral reasoning ability of LLMs using the Defining Issues Test - a psychometric instrument developed for measuring the moral development stage of a person according to the Kohlberg's Cognitive Moral Development Model. DIT uses moral dilemmas followed by a set of ethical considerations that the respondent has to judge for importance in resolving the dilemma, and then rank-order them by importance. A moral development stage score of the respondent is then computed based on the relevance rating and ranking. Our study shows that early LLMs such as GPT-3 exhibit a moral reasoning ability no better than that of a random baseline, while ChatGPT, Llama2-Chat, PaLM-2 and GPT-4 show significantly better performance on this task, comparable to adult humans. GPT-4, in fact, has the highest post-conventional moral reasoning score, equivalent to that of typical graduate school students. However, we also observe that the models do not perform consistently across all dilemmas, pointing to important gaps in their understanding and reasoning abilities.

==> background.tex <==
F\section{Background/Primer on Moral Theories of Philosophy}

Morality is the study that deals with what is right or wrong and has been a central concern in philosophy. Over the years, numerous theories have emerged to explain how individuals develop their moral reasoning and judgments. This section will delve into some prominent moral theories, beginning with Piaget's law and progressing through Kohlberg's Theory, Ruest's Defining Issues Test (DIT), and more contemporary ones like Moral foundation Theory and Dual Process Theory.

\subsection{Piaget's Law of Moral Development}
Piaget's theory (1932) focuses on the cognitive aspects of morality, proposing that moral reasoning evolves through stages of cognitive development\cite{piaget2013moral}. Jean Piaget argued that children progress from a stage of moral realism, where they adhere strictly to rules and authority, to a stage of moral relativism, where they begin to consider different perspectives and understand that rules can be flexible. He proposed four development stages: sensorimotor stage (Birth to 2 years), preoperational stage (2 to 7 years), concrete operational stage (7 to 11 years), and four operation stage (Adolescence and Beyond). This theory faced some criticisms like setting rigid age-based stages, lack of emphasis on social and cultural contexts, and limited attention to emotional development.

\subsection{Kohlberg's Theory of Moral Development}
Building upon Piaget's work, Lawrence Kohlberg developed a comprehensive theory of moral development known as Cognitive Moral Development (CMD) model \cite{KohlbergCMD} in 1969. Kohlberg's theory consists of six stages divided into three main levels: pre-conventional, conventional, and post-conventional morality as shown in Figure~\ref{fig:CMD}. In Stage 1, individuals are concerned with avoiding punishment and make moral decisions based on fear of consequences and self-interest. At Stage 2, individuals focus on their own needs and interests but recognize that others have similar needs. Moral judgments are influenced by reciprocity, such as "You scratch my back, I'll scratch yours. At Stage 3, individuals seek approval and conform to social norms. Moral decisions are made to maintain positive relation ships and avoid disapproval. At stage 4, individuals are concerned with law, rules, and authority figures and their moral reasoning revolves around maintaining social order and upholding the greater good. At Stage 5, individuals recognize different groups may have different moral perspectives and base their decisions on principles of fairness, justice, and individual rights, even if these principles conflict with social norms or laws. At stage 6, individuals develop their moral principles based on universal ethical values. They act according to a personal ethical code that transcends societal rules and laws. These principles often align with concepts of justice, equality, and human rights. This theory emphasizes the importance of moral reasoning and the development of an individual's moral principles. It posits that as individuals mature, their moral reasoning becomes more sophisticated and abstract, allowing them to make ethical decisions based on principles rather than mere rules. This theory also faced criticisms such as stages' bias towards Western, Individualistic cultures, hence overlooking the diversity of moral development across cultures \cite{dien1982chinese, snarey1985cross}, having gender bias \cite{bebeau1987integrating}, lacking considerations of emotions, intuitions or the role of emotions in moral decision making \cite{haidt2001emotional}.  Despite these, Kohlberg's theory has played a vital role in advancing our understanding of moral development and remains influential in the field of moral psychology.

% \indent
% \begin{figure}
%  \centering
%  \includegraphics[scale=0.4]{CMD.png}
%  \caption{The six stages of CMD according to Kohlberg}
%  \label{fig:CMD}
% \end{figure}


\subsection{Rest's Defining Issues Test}
In line with Kohlberg's framework, James Rest introduced the Defining Issues Test (DIT) \cite{Rest1986A} as a way to measure an individual's moral development. DIT progresses from an egocentric perspective on moral issues to a collective moral viewpoint and ultimately relies on post-conventional moral principles. The DIT presents respondents with moral dilemmas and assesses their moral reasoning by analyzing the justifications provided for their decisions. Rest's DIT draws upon Kohlberg's stages to categorize individuals into stages of moral development, offering insights into ethical decision-making processes. For over three decades, the DIT has remained the most popular tool for assessing CMD. It includes either three (short-form DIT) or six (original DIT) moral dilemmas, each followed by 12 statements corresponding to different CMD stages. Participants rate the significance of each statement in ethical judgment and then select and rank the four most important statements.

The Post Conventional Morality Score (abbreviated as P-score), stands as the most widely utilized metric, serving as an indicator of the "relative significance an individual places on principled moral considerations, specifically those associated with Stages five and six, when deliberating moral dilemmas" \cite{rest1990dit}. This score, which spans from 0 to 95, is determined by assigning points to the four most pivotal statements chosen by the individual, aligning with Stages 5 and 6 of Cognitive Moral Development (CMD). The most vital statement corresponding to either Stage 5 or 6 receives four points, the second most crucial statement related to either Stage 5 or 6 earns three points, and so forth. P-score tends to focus on these considerations that include adhering to decisions made by the majority, ensuring the fair implementation of established procedures, and safeguarding fundamental rights. Apart from P-score, DIT also measure Personal Interest Schema Score which reflects choices influenced by personal interests (Stages 2 and 3 in Kohlberg's model), such as direct benefits, fairness, intentions, relationship concerns, and approval. Maintaining Norms Schema Score indicates choices driven by societal norms, including legal systems, established roles, and organizational structures. The percentage of "Can't Decide" Choices measures the respondent's decisiveness in selecting options. It calculates how often the "can't decide" option is chosen, reflecting the ease of processing moral information.


\subsection{Recent Theories in Moral Philosophy}
In recent years, moral philosophy has seen the emergence of innovative theories that expand our understanding of moral decision-making developed by social psychologists. Moral Foundations Theory proposed by Jonathan Haidt and Jesse Graham, posits that human morality is shaped by a set of innate moral foundations or intuitions \cite{graham2013moral}. These foundations include care/harm, fairness/cheating, loyalty/betrayal, authority/subversion, and sanctity/degradation. According to this theory, individuals vary in the extent to which they prioritize these moral foundations, leading to differences in moral judgments and values. Dual Process Theory, rooted in psychology and neuroscience, posits that moral decision-making involves two cognitive processes: System 1 (intuitive) and System 2 (reflective) \cite{tam2022evaluating}. System 1 operates quickly and automatically, relying on gut feelings and emotions, while System 2 involves deliberate reasoning and critical thinking. This theory suggests that moral judgments often result from the interplay between these two systems, and the balance can vary among individuals and situations. 



% \subsection{Kohlberg's Theory of Moral Development}
% The Cognitive Moral Development (CMD) model proposed by Kohlberg in 1969 has had a significant influence on the domain of ethics research \cite{KohlbergCMD}. The premise of this notion is that individuals undergo a developmental process in their moral reasoning from infancy to adulthood. According to Rest's (1979) \cite{rest1979development} theory, CMD entails the development of moral reasoning and a subsequent elevation to a more sophisticated stage that denotes an enhanced comprehension of the ethical responsibilities within complex social systems. The six distinct stages of Cognitive Moral Development (CMD) are classified into three broad stages, namely pre-conventional, conventional, and post-conventional. As shown in Figure~\ref{fig:CMD}, Kohlberg proposed six stages of CMD that can be grouped into three levels Kohlberg's theory posits that the pre-conventional Stages 1 and 2 are commonly observed in young children, whereas the conventional Stages 3 and 4 are predominantly exhibited by adults.
% Merely a minority of the adult populace, ranging from 20\% to 25\%, attains the ultimate two post-conventional stages.
% The stages of CMD theory are indicative of different ways of thinking for approaching moral questions. Individuals at the pre-conventional level perceive themselves as valuing interpersonal relationships solely as a means to fulfill their own needs. During the conventional stages of development, individuals tend to identify themselves as integral components of their immediate social environment. As a result, they often strive to conform to stereotypical behavioral norms that are commonly shared among members of their community. The behaviors deemed appropriate by these individuals are those that align with the values held by the majority. At the post-conventional stage of moral development, individuals prioritize social order beyond their immediate social circle due to their profound reverence for the rights of others.



% The initial argument posited by CMD was that there exists a correlation between moral development and subsequent moral actions, as previously noted by Colby and Kohlberg in 1984 \cite{Colby_undated-yh}. Presently, it is widely agreed upon that Cognitive Moral Development (CMD) is a prerequisite for ethical behavior, albeit not a comprehensive one, as posited by Kohlberg (1969) \cite{KohlbergCMD} and Rest (1979) \cite{rest1979development}. Despite variations in findings, scholars have generally established a favorable correlation between Cognitive Moral Development (CMD) and ethical conduct, as evidenced by Rest (1986a) \cite{Rest1986A} and subsequent studies such as Gooslby and Hunt (1992) \cite{Goolsby1992CognitiveMD}.

% \subsection{DIT Framework}
% In line with Kohlberg's framework, Rest saw moral judgment development as a social and cognitive process. It progresses from an egocentric perspective on moral issues to a collective moral viewpoint and ultimately relies on post-conventional moral principles. Rest also shared Kohlberg's view that moral judgments are primarily cognitive and play a central role in understanding moral actions and emotions.

% The Defining Issues Test (DIT) is firmly rooted in Kohlberg's moral development theory and encompasses all six stages of Cognitive Moral Development (CMD) \cite{rest1979development}. The DIT employs a unique rating and ranking task to understand how individuals interpret moral situations. It supports a developmental model where growth involves a gradual shift toward more complex conceptions of social and moral cooperation.

% What sets the DIT apart is its innovative data collection approach. Unlike Kohlberg's time-consuming Moral Judgment Interview (MJI), the DIT uses a user-friendly multiple-choice questionnaire format, making it easier to administer. By 1986, over 500 studies from more than 20 countries had utilized the DIT \cite{Rest1986A}.

% For over three decades, the DIT has remained the most popular tool for assessing CMD. It includes either three (short-form DIT) or six (original DIT) moral dilemmas, each followed by 12 statements corresponding to different CMD stages. Participants rate the significance of each statement in ethical judgment and then select and rank the four most important statements. 

% \subsection{DIT Scoring and Indices and their interpretations}
% The Post Conventional Morality Score (abbreviated as P-score), stands as the most widely utilized metric, serving as an indicator of the "relative significance an individual places on principled moral considerations, specifically those associated with Stages five and six, when deliberating moral dilemmas" \cite{rest1990dit}. This score, which spans from 0 to 95, is determined by assigning points to the four most pivotal statements chosen by the individual, aligning with Stages 5 and 6 of Cognitive Moral Development (CMD). The most vital statement corresponding to either Stage 5 or 6 receives four points, the second most crucial statement related to either Stage 5 or 6 earns three points, and so forth. P-score tends to focus on these considerations that include adhering to decisions made by the majority, ensuring the fair implementation of established procedures, and safeguarding fundamental rights.

% Apart from P-score, DIT also measure Personal Interest Schema Score which reflects choices influenced by personal interests (Stages 2 and 3 in Kohlberg's model), such as direct benefits, fairness, intentions, relationship concerns, and approval. Maintaining Norms Schema Score indicates choices driven by societal norms, including legal systems, established roles, and organizational structures. The percentage of "Can't Decide" Choices measures the respondent's decisiveness in selecting options. It calculates how often the "can't decide" option is chosen, reflecting the ease of processing moral information.

% \subsection{Criticisms of DIT}
% The DIT primarily focuses on formal moral reasoning, which is the ability to engage in abstract ethical reasoning and is based on Kohlberg's theory of moral development. Critics argue that this narrow focus overlooks other important aspects of moral behavior, such as emotions, intuitions, and cultural variations in moral values.

% The DIT was developed in a Western cultural context, and its scenarios and dilemmas may not be relevant or appropriate for individuals from non-Western cultures. This cultural bias can limit its applicability and accuracy in assessing moral development in diverse populations. In this study, we have also curated new dilemmas which covers up the the scenarios of non-Western society to mitigate this cultural bias. 

% Despite these criticisms, the DIT remains a valuable tool for assessing moral reasoning and measuring CMD and has contributed significantly to the field of moral psychology. Researchers continue to refine and adapt the instrument to address some of these limitations and expand its applicability to diverse populations and contexts.
